Analytical solutions for the Extracellular-Membrane-Intracellular model

The Extracellular-Membrane-Intracellular (EMI) model is a novel mathematical framework for cardiac electrophysiology simulations. The EMI model provides a more detailed description of the heart's electrical activity compared to traditional monodomain and bidomain models, potentially making it better-suited for understanding the electrical dynamics of the heart under pathological conditions. In this paper, we derive and verify several analytical solutions for the EMI model. Specifically, we obtain a family of solutions for a single two-dimensional cell in polar coordinates and for a pair of coupled three-dimensional cells in spherical coordinates. We also introduce a manufactured solution for N three-dimensional cells in Cartesian coordinates. To verify the analytical solutions, we conduct numerical experiments using the mortar finite element method combined with operator splitting. The results demonstrate that the analytical solutions are effective for verifying the accuracy of numerical simulations of the EMI model.

==> images/fig-EMI-model.tex <==
\begin{figure}[H]
\centering
\resizebox{0.6\textwidth}{!}{%


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Rounded Rect [id:dp2448998471028715] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=1.5]  (211.28,60.9) .. controls (211.28,52.2) and (218.33,45.14) .. (227.03,45.14) -- (475.79,45.14) .. controls (484.49,45.14) and (491.54,52.2) .. (491.54,60.9) -- (491.54,267.59) .. controls (491.54,276.29) and (484.49,283.34) .. (475.79,283.34) -- (227.03,283.34) .. controls (218.33,283.34) and (211.28,276.29) .. (211.28,267.59) -- cycle ;
%Shape: Path Data [id:dp01602773270414437] 
\draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (279.99,163.91) -- (279.99,143.69) -- (249.77,143.69) -- (249.93,123.41) -- (229.93,123.41) -- (229.93,103.63) -- (249.75,103.63) -- (249.93,83.41) -- (279.6,83.41) -- (279.6,64.05) -- (299.77,64.05) -- (299.77,83.47) -- (330.43,83.47) -- (330.43,103.69) -- (370,103.69) -- (369.99,83.47) -- (399.66,83.47) -- (399.66,64.11) -- (419.82,64.11) -- (419.82,83.52) -- (450.49,83.52) -- (450.49,103.74) -- (470.04,103.74) -- (470.04,123.52) -- (450.49,123.52) -- (450.49,143.52) -- (420.27,143.3) -- (420.27,163.97) -- (420.21,163.97) -- (420.21,183.38) -- (450.88,183.38) -- (450.88,203.61) -- (470.43,203.61) -- (470.43,223.38) -- (450.88,223.38) -- (450.88,243.38) -- (420.66,243.16) -- (420.66,263.83) -- (400.43,263.83) -- (400.43,243.61) -- (370.21,243.61) -- (370.38,223.33) -- (330.88,223.33) -- (330.88,243.33) -- (300.66,243.11) -- (300.66,263.77) -- (280.43,263.77) -- (280.43,243.55) -- (250.21,243.55) -- (250.38,223.27) -- (230.38,223.27) -- (230.38,203.63) -- (250.25,203.63) -- (250.38,183.27) -- (280.04,183.27) -- (280.04,163.91) -- (279.99,163.91) -- cycle (330.43,123.47) -- (330.43,143.47) -- (300.21,143.24) -- (300.21,183.33) -- (330.88,183.33) -- (330.88,203.55) -- (370.19,203.55) -- (370.38,183.33) -- (400.04,183.33) -- (400.04,143.74) -- (369.82,143.74) -- (369.99,123.47) -- (330.43,123.47) -- cycle ;
%Straight Lines [id:da19655730385405767] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (299.14,163.91) -- (281.18,163.91) ;
%Straight Lines [id:da7840217471929752] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (419.14,163.97) -- (405.72,163.97) -- (401.14,163.97) ;
%Straight Lines [id:da3572310995825507] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (350.43,204.64) -- (350.43,222.21) ;
%Straight Lines [id:da11642707835768351] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=1.5]    (349.85,104.79) -- (349.85,122.5) ;
%Curve Lines [id:da7478236039212312] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ]   (267.6,159.1) .. controls (274.1,154.65) and (287.4,156.7) .. (290.13,163.91) ;
%Curve Lines [id:da4354733762740608] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ]   (410.16,163.97) .. controls (412.75,155.13) and (427.5,152.88) .. (432,157.38) ;
%Curve Lines [id:da7476297495183056] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=0.75]    (348,233.88) .. controls (341.25,227.88) and (343,216.38) .. (350.43,213.11) ;
%Curve Lines [id:da4779988569681656] 
\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=0.75]    (347.56,134.01) .. controls (340.81,128.01) and (342.56,116.51) .. (349.99,113.24) ;


% Text Node
\draw (428.95,32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\Gammae $};
% Text Node
\draw (282.17,102.23) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\Omegai[1] $};
% Text Node
\draw (402.17,102.73) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\Omegai[2] $};
% Text Node
\draw (402.33,202.57) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\Omegai[4] $};
% Text Node
\draw (282.33,202.07) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\Omegai[3] $};
% Text Node
\draw (345.2,63.2) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\Omegae $};
% Text Node
\draw (335,135) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\GammaGap[1,2] $};
% Text Node
\draw (425,160) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\GammaGap[2,4] $};
% Text Node
\draw (335,235) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\GammaGap[3,4] $};
% Text Node
\draw (245,160) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\GammaGap[1,3] $};
% Text Node
\draw (426.08,63) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\Gammai[2] $};
% Text Node
\draw (251.17,63) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\Gammai[1] $};
% Text Node
\draw (425.25,246) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\Gammai[4] $};
% Text Node
\draw (249.83,246) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\Gammai[3] $};


\end{tikzpicture}

}%
\caption{Configuration of a two-dimensional domain with four cells (purple) surrounded by extracellular space (blue) with gap junctions (orange) \cite{Tveito2017}.}
\label{fig:EMI_Model}
\end{figure}

==> images/fig-Manufactured-solutions.tex <==
\begin{figure}[htbp]
    \centering  
    \subfigure[$xy$-plane representation of the single cell.]
    {  
    \resizebox{0.45\textwidth}{!}{%

    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
    %uncomment if require: \path (0,422); %set diagram left start at 0, and has height of 422
    
    %Straight Lines [id:da5551921308039518] 
    \draw    (150.78,334.8) -- (449.94,334.89) ;
    \draw [shift={(449.94,334.89)}, rotate = 180.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(150.78,334.8)}, rotate = 180.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Straight Lines [id:da08538486398188716] 
    \draw    (275.9,55.56) -- (325.4,55.56) ;
    \draw [shift={(325.4,55.56)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(275.9,55.56)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Straight Lines [id:da8129584704329456] 
    \draw    (128.43,313.7) -- (129.1,75.2) ;
    \draw [shift={(129.1,75.2)}, rotate = 90.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(128.43,313.7)}, rotate = 90.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Straight Lines [id:da5565153731642678] 
    \draw    (399.98,105.06) -- (449.48,105.06) ;
    \draw [shift={(449.48,105.06)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(399.98,105.06)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Straight Lines [id:da3715330092574036] 
    \draw    (180.2,75.6) -- (180.2,125.1) ;
    \draw [shift={(180.2,125.1)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(180.2,75.6)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Shape: Rectangle [id:dp941816063685415] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ][line width=1.5]  (200.2,125.5) -- (400.2,125.5) -- (400.2,265) -- (200.2,265) -- cycle ;
    %Shape: Square [id:dp6137265481471254] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ][line width=1.5]  (275.9,76) -- (325.4,76) -- (325.4,125.5) -- (275.9,125.5) -- cycle ;
    %Shape: Square [id:dp4424210648642707] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ][line width=1.5]  (400.31,170.59) -- (449.81,170.59) -- (449.81,220.09) -- (400.31,220.09) -- cycle ;
    %Shape: Square [id:dp2730149613878048] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ][line width=1.5]  (150.65,170.5) -- (200.15,170.5) -- (200.15,220) -- (150.65,220) -- cycle ;
    %Shape: Square [id:dp41475321381402186] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ][line width=1.5]  (275.23,265) -- (324.73,265) -- (324.73,314.5) -- (275.23,314.5) -- cycle ;
    
    %Straight Lines [id:da3704444402697785] 
    \draw    (470.64,170.93) -- (470.64,220.43) ;
    \draw [shift={(470.64,220.43)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(470.64,170.93)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Shape: Rectangle [id:dp304292246755396] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (201.6,124.5) -- (401.6,124.5) -- (401.6,264) -- (201.6,264) -- cycle ;
    %Shape: Square [id:dp999808258845248] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (277.3,75) -- (326.8,75) -- (326.8,124.5) -- (277.3,124.5) -- cycle ;
    %Shape: Square [id:dp3217396061361558] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (401.71,169.59) -- (451.21,169.59) -- (451.21,219.09) -- (401.71,219.09) -- cycle ;
    %Shape: Square [id:dp8898709915249071] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (152.05,169.5) -- (201.55,169.5) -- (201.55,219) -- (152.05,219) -- cycle ;
    %Shape: Square [id:dp8955087984831451] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (276.63,264) -- (326.13,264) -- (326.13,313.5) -- (276.63,313.5) -- cycle ;
    
    %Straight Lines [id:da8898244407492027] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (451.21,169.59) -- (451.21,219.09) ;
    %Straight Lines [id:da49871862180133053] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (277.3,75) -- (326.8,75) ;
    %Straight Lines [id:da184592383184912] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (152.05,169.5) -- (152.05,219) ;
    %Straight Lines [id:da6734435180627456] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (276.63,313.5) -- (326.13,313.5) ;
    
    % Text Node
    \draw (293,340) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\alpha _{c}$};
    % Text Node
    \draw (100,185) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\beta _{c}$};
    % Text Node
    \draw (415.11,78) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\alpha _{g}$};
    % Text Node
    \draw (150.73,87.6) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\beta _{g}$};
    % Text Node
    \draw (293,28.62) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\alpha _{g}$};
    % Text Node
    \draw (474.98,185) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\beta _{g}$};
    
    
    \end{tikzpicture}
    


    }%
    
    }  
    \hfill
    % The only difference is here, where I have commented out an empty line.
    \subfigure[$yz$-plane representation of the single cell.]  
    {      

    \resizebox{0.4\textwidth}{!}{%



    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
    %uncomment if require: \path (0,422); %set diagram left start at 0, and has height of 422
    
    %Shape: Rectangle [id:dp05220277883045232] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=0.75]  (224.2,127.83) -- (356,127.83) -- (356,267.33) -- (224.2,267.33) -- cycle ;
    %Shape: Square [id:dp6834712664135474] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=0.75]  (174.64,172.59) -- (224.14,172.59) -- (224.14,222.09) -- (174.64,222.09) -- cycle ;
    %Shape: Square [id:dp23092653810014707] 
    \draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=0.75]  (355.97,172.26) -- (405.47,172.26) -- (405.47,221.76) -- (355.97,221.76) -- cycle ;
    
    %Shape: Square [id:dp07892734441635152] 
    \draw  [draw opacity=0][line width=1.5]  (265.35,172.83) -- (314.85,172.83) -- (314.85,222.33) -- (265.35,222.33) -- cycle ;
    %Straight Lines [id:da5513158064659619] 
    \draw    (153.53,267.33) -- (153.53,127.83) ;
    \draw [shift={(153.53,127.83)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(153.53,267.33)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Straight Lines [id:da9053094724303927] 
    \draw    (424.81,222.43) -- (424.81,172.93) ;
    \draw [shift={(424.81,172.93)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    \draw [shift={(424.81,222.43)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
    %Shape: Rectangle [id:dp4899532936764398] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (225.12,126.91) -- (356.92,126.91) -- (356.92,266.41) -- (225.12,266.41) -- cycle ;
    %Shape: Square [id:dp1524891758851551] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (175.56,171.67) -- (225.06,171.67) -- (225.06,221.17) -- (175.56,221.17) -- cycle ;
    %Shape: Square [id:dp7483509984718204] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=1.5]  (356.9,171.34) -- (406.4,171.34) -- (406.4,220.84) -- (356.9,220.84) -- cycle ;
    
    %Shape: Polygon [id:ds18029193276306354] 
    \draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]  (320.6,171.7) -- (271.1,171.7) -- (271.1,221.2) -- (320.6,221.2) -- cycle ;
    %Straight Lines [id:da5438309978250423] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (175.24,222.09) -- (175.24,172.59) ;
    %Straight Lines [id:da2061269837422497] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=2.25]    (406.4,220.84) -- (406.4,171.34) ;
    
    %Shape: Rectangle [id:dp9612264145734605] 
    \draw  [draw opacity=0] (135.28,36.58) -- (453.1,36.58) -- (453.1,343.5) -- (135.28,343.5) -- cycle ;
    
    % Text Node
    \draw (125.98,189) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\gamma _{c}$};
    % Text Node
    \draw (431.98,189) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\gamma _{g}$};
    
    
    \end{tikzpicture}
    
    
    }%  
    }
    \caption{Single three-dimensional cardiac cell and its dimensions:
      cell membranes (purple) and gap junctions (orange).}
    \label{fig:manufactured-solutions}
    \end{figure}

==> images/fig-Single-cell.tex <==
\begin{figure}[H]
    \centering
    \resizebox{0.43\textwidth}{!}{%
    
    
    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
    
    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
    %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
    
    %Shape: Circle [id:dp473609368365674] 
    \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=2.25]  (202.8,150.45) .. controls (202.8,80.17) and (259.77,23.2) .. (330.05,23.2) .. controls (400.33,23.2) and (457.3,80.17) .. (457.3,150.45) .. controls (457.3,220.73) and (400.33,277.7) .. (330.05,277.7) .. controls (259.77,277.7) and (202.8,220.73) .. (202.8,150.45) -- cycle ;
    %Shape: Circle [id:dp40200735952364375] 
    \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=2.25]  (253.05,150.45) .. controls (253.05,107.92) and (287.52,73.45) .. (330.05,73.45) .. controls (372.58,73.45) and (407.05,107.92) .. (407.05,150.45) .. controls (407.05,192.98) and (372.58,227.45) .. (330.05,227.45) .. controls (287.52,227.45) and (253.05,192.98) .. (253.05,150.45) -- cycle ;
    %Straight Lines [id:da5342875233556422] 
    \draw    (330.05,150.45) -- (516.3,150.45) ;
    \draw [shift={(519.3,150.45)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
    \draw [shift={(330.05,150.45)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.68, y radius= 2.68]   ;
    %Straight Lines [id:da5650247282127798] 
    \draw    (369.41,111.19) -- (398.49,82.11) ;
    \draw [shift={(399.9,80.7)}, rotate = 135] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
    \draw [shift={(368,112.6)}, rotate = 315] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
    %Straight Lines [id:da8293120914452778] 
    \draw    (420.2,59.9) -- (435.59,44.51) ;
    \draw [shift={(437,43.1)}, rotate = 135] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
    
    % Text Node
    \draw (221.5,34.9) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Gammae $};
    % Text Node
    \draw (254,68) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Gammai[1] $};
    % Text Node
    \draw (279.5,167.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Omegai[1] $};
    % Text Node
    \draw (242,205.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Omegae $};
    % Text Node
    \draw (349,83.9) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nex$};
    % Text Node
    \draw (372,55) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nin[1] $};
    % Text Node
    \draw (410,22) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nex$};
    % Text Node
    \draw (325.05,158.55) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$0$};
    % Text Node
    \draw (410.55,157.85) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$r_{1}$};
    % Text Node
    \draw (460.8,157.35) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$r_{2}$};
    % Text Node
    \draw (506.55,157.6) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$r$};
    
    
    \end{tikzpicture}
    
    
    }%
    \caption{Domain representation for a single circular cell (purple) surrounded by a circular layer as extracellular space (blue).}
    \label{fig:one_spherical_cell}
    \end{figure}

==> images/fig-Two-coupled-cells.tex <==
\begin{figure}[htbp]
    \centering  
    \subfigure[Three-dimensional representation of two coupled
    semi-spherical cells.]
    {  
    \resizebox{0.35\textwidth}{!}{%

        % Gradient Info
        
        \tikzset {_zj14x22i8/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{-198 bp } { 158.4 bp }  }  \pgftransformscale{1.32 }  }}}
        \pgfdeclareradialshading{_2q0j731r4}{\pgfpoint{160bp}{-128bp}}{rgb(0bp)=(1,1,1);
        rgb(0bp)=(1,1,1);
        rgb(25bp)=(0.29,0.56,0.89);
        rgb(400bp)=(0.29,0.56,0.89)}

        % Gradient Info
        
        \tikzset {_7be5t0jos/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformscale{1 }  }}}
        \pgfdeclareradialshading{_zwhalcii7}{\pgfpoint{0bp}{0bp}}{rgb(0bp)=(0.98,0.98,0.98);
        rgb(0.26785714285714285bp)=(0.98,0.98,0.98);
        rgb(25bp)=(0.29,0.56,0.89);
        rgb(400bp)=(0.29,0.56,0.89)}

        % Gradient Info
        
        \tikzset {_gz8tbg6ow/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformscale{1 }  }}}
        \pgfdeclareradialshading{_gvz3gg555}{\pgfpoint{0bp}{0bp}}{rgb(0bp)=(0.97,0.47,0.89);
        rgb(0bp)=(0.97,0.47,0.89);
        rgb(25bp)=(0.74,0.06,0.88);
        rgb(400bp)=(0.74,0.06,0.88)}

        % Gradient Info
        
        \tikzset {_pu6dsamcu/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{-198 bp } { 158.4 bp }  }  \pgftransformscale{1.32 }  }}}
        \pgfdeclareradialshading{_28pqi3i1o}{\pgfpoint{160bp}{-128bp}}{rgb(0bp)=(1,1,1);
        rgb(0bp)=(1,1,1);
        rgb(25bp)=(0.29,0.56,0.89);
        rgb(400bp)=(0.29,0.56,0.89)}
        \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

        \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
        %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

        %Shape: Chord [id:dp6281688393363907] 
        \draw  [draw opacity=0][shading=_2q0j731r4,_zj14x22i8] (438.72,178.71) .. controls (438.73,179.66) and (438.74,180.62) .. (438.73,181.58) .. controls (438.26,240.63) and (388.49,288.1) .. (327.58,287.61) .. controls (266.67,287.13) and (217.67,238.86) .. (218.15,179.8) .. controls (218.16,179.05) and (218.17,178.3) .. (218.19,177.55) -- cycle ;
        %Shape: Ellipse [id:dp7912340229173132] 
        \draw  [draw opacity=0][shading=_zwhalcii7,_7be5t0jos] (218.16,178.88) .. controls (218.16,163.9) and (267.53,151.75) .. (328.44,151.75) .. controls (389.34,151.75) and (438.71,163.9) .. (438.71,178.88) .. controls (438.71,193.87) and (389.34,206.02) .. (328.44,206.02) .. controls (267.53,206.02) and (218.16,193.87) .. (218.16,178.88) -- cycle ;
        %Shape: Ellipse [id:dp707186947722418] 
        \path  [shading=_gvz3gg555,_gz8tbg6ow] (259.99,179.66) .. controls (259.99,170.35) and (290.63,162.81) .. (328.44,162.81) .. controls (366.24,162.81) and (396.88,170.35) .. (396.88,179.66) .. controls (396.88,188.96) and (366.24,196.5) .. (328.44,196.5) .. controls (290.63,196.5) and (259.99,188.96) .. (259.99,179.66) -- cycle ; % for fading 
        \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ] (259.99,179.66) .. controls (259.99,170.35) and (290.63,162.81) .. (328.44,162.81) .. controls (366.24,162.81) and (396.88,170.35) .. (396.88,179.66) .. controls (396.88,188.96) and (366.24,196.5) .. (328.44,196.5) .. controls (290.63,196.5) and (259.99,188.96) .. (259.99,179.66) -- cycle ; % for border 

        %Shape: Path Data [id:dp30289798692772707] 
        \draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]  (321.07,196.38) .. controls (320.51,196.39) and (319.96,196.38) .. (319.42,196.34) -- (335.83,162.87) .. controls (336.39,162.88) and (336.94,162.88) .. (337.49,162.89) -- (321.07,196.38) -- cycle ;

        %Shape: Path Data [id:dp6243706793920073] 
        \draw  [draw opacity=0][shading=_28pqi3i1o,_pu6dsamcu] (216.41,112.07) .. controls (217.25,52.28) and (267.3,4.5) .. (328.21,5.35) .. controls (389.13,6.2) and (437.83,55.36) .. (436.99,115.15) .. controls (436.99,115.47) and (436.98,115.78) .. (436.98,116.1) .. controls (436.98,131.08) and (387.6,143.23) .. (326.7,143.23) .. controls (266.97,143.23) and (218.33,131.55) .. (216.47,116.96) -- (216.45,116.96) .. controls (216.45,116.87) and (216.45,116.78) .. (216.44,116.69) .. controls (216.43,116.5) and (216.42,116.3) .. (216.42,116.1) .. controls (216.42,116.01) and (216.42,115.92) .. (216.42,115.84) .. controls (216.4,114.59) and (216.39,113.33) .. (216.41,112.07) -- cycle ;
        \end{tikzpicture}

    }%
    
    }  
    \hfill
    % The only difference is here, where I have commented out an empty line.
    \subfigure[Two-dimensional cross-section of two semi-spherical cells.]  
    {      

    \resizebox{0.45\textwidth}{!}{%
        \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

        \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
        %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
        
        %Shape: Circle [id:dp182949511535212] 
        \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.1 ][line width=2.25]  (223.47,149.42) .. controls (223.47,79.14) and (280.44,22.17) .. (350.72,22.17) .. controls (420.99,22.17) and (477.97,79.14) .. (477.97,149.42) .. controls (477.97,219.69) and (420.99,276.67) .. (350.72,276.67) .. controls (280.44,276.67) and (223.47,219.69) .. (223.47,149.42) -- cycle ;
        %Shape: Circle [id:dp31473887829507285] 
        \draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.1 ][line width=2.25]  (273.72,149.42) .. controls (273.72,106.89) and (308.19,72.42) .. (350.72,72.42) .. controls (393.24,72.42) and (427.72,106.89) .. (427.72,149.42) .. controls (427.72,191.94) and (393.24,226.42) .. (350.72,226.42) .. controls (308.19,226.42) and (273.72,191.94) .. (273.72,149.42) -- cycle ;
        %Straight Lines [id:da48692514763043093] 
        \draw    (390.08,110.15) -- (419.15,81.08) ;
        \draw [shift={(420.57,79.67)}, rotate = 135] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
        \draw [shift={(388.67,111.57)}, rotate = 315] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
        %Straight Lines [id:da6395541981301534] 
        \draw    (440.87,58.87) -- (456.25,43.48) ;
        \draw [shift={(457.67,42.07)}, rotate = 135] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
        %Straight Lines [id:da40913045120902136] 
        \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=3]    (350.72,72.42) -- (350.72,226.42) ;
        %Straight Lines [id:da5569673303366386] 
        \draw    (350.72,149.42) -- (536.97,149.42) ;
        \draw [shift={(539.97,149.42)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
        \draw [shift={(350.72,149.42)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.68, y radius= 2.68]   ;
        %Straight Lines [id:da8678355911609739] 
        \draw    (370.67,136.5) -- (329,136.5) ;
        \draw [shift={(327,136.5)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
        \draw [shift={(372.67,136.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (9.6,-2.4) -- (0,0) -- (9.6,2.4) -- cycle    ;
        
        % Text Node
        \draw (242.17,33.87) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Gammae $};
        % Text Node
        \draw (402.33,210) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Gammai[2] $};
        % Text Node
        \draw (305.83,175.7) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Omegai[1] $};
        % Text Node
        \draw (240,133.03) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Omegae $};
        % Text Node
        \draw (369.67,82.87) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nex $};
        % Text Node
        \draw (393,55) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nin[2] $};
        % Text Node
        \draw (434,24) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nex $};
        % Text Node
        \draw (352.72,152.82) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$0$};
        % Text Node
        \draw (431.22,156.82) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\rho_{1}$};
        % Text Node
        \draw (481.47,156.32) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\rho_{2}$};
        % Text Node
        \draw (527.22,156.57) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\rho$};
        % Text Node
        \draw (360.83,175.37) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Omegai[2] $};
        % Text Node
        \draw (270,210) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Gammai[1] $};
        % Text Node
        \draw (376.05,120) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nin[1] $};
        % Text Node
        \draw (296,120) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\nin[2] $};
        \end{tikzpicture}
    
    }%  
    }
    \caption{Domain representation of two coupled semi-spherical cells (purple) 
    connected by a gap junction (orange) and surrounded by a spherical 
    shell-shaped extracellular space (blue).} 
    \label{fig:two_semispherical_cells}
    \end{figure}
